A moment-matching Ferguson and Klass algorithm

Completely random measures (CRM) represent the key building block of a wide variety of popular stochastic models and play a pivotal role in modern Bayesian Nonparametrics. A popular representation of CRMs as a random series with decreasing jumps is due to Ferguson and Klass (1972). This can immediately be turned into an algorithm for sampling realizations of CRMs or more elaborate models involving transformed CRMs. However, concrete implementation requires to truncate the random series at some threshold resulting in an approximation error. The goal of this paper is to quantify the quality of the approximation by a moment-matching criterion, which consists in evaluating a measure of discrepancy between actual moments and moments based on the simulation output. Seen as a function of the truncation level, the methodology can be used to determine the truncation level needed to reach a certain level of precision. The resulting moment-matching \FK algorithm is then implemented and illustrated on several popular Bayesian nonparametric models.

==> paper for arxiv/tab_galaxy.tex <==
%\begin{center}
\begin{table}[ht!]
\begin{center}
\begin{tabular}{lccc}
\toprule
$\gamma$& $e_M = 0.1$ & $e_M = 0.05$ & $e_M = 0.01$ \\
  \hline %\\[-0.3cm]
$0$ & 19.4 & 15.5 & 9.2 \\
$0.25$ & 31.3 & 23.7 & 15.1 \\
$0.5$ & 42.4  & 28.9 & 18.3 \\
$0.75$ & 64.8 & 41.0 & 23.2 \\
\bottomrule
\end{tabular}
\end{center}
\caption{\label{tab:galaxy} \texttt{Galaxy} dataset. Kolmogorov--Smirnov distance $d_{KS}(\hat F_{\ell_M}, \hat F_{e_M})$ between estimated cdfs $\hat F_{\ell_M}$ and $\hat F_{e_M}$ under, respectively, the moment-match (with $\ell_M = 0.01$) and the relative error (with $e_M = 0.1, 0.05, 0.01$) criteria. The mixing measure of normal mixture is the \NGG with varying $\gamma\in\{0,0.25,0.5,0.75\}$.}
\end{table}
%\end{center} 

==> tab_galaxy.tex <==
%\begin{center}
\begin{table}[ht!]
\begin{center}
\begin{tabular}{lccc}
\toprule
$\gamma$& $e_M = 0.1$ & $e_M = 0.05$ & $e_M = 0.01$ \\
  \hline %\\[-0.3cm]
$0$ & 19.4 & 15.5 & 9.2 \\
$0.25$ & 31.3 & 23.7 & 15.1 \\
$0.5$ & 42.4  & 28.9 & 18.3 \\
$0.75$ & 64.8 & 41.0 & 23.2 \\
\bottomrule
\end{tabular}
\end{center}
\caption{\label{tab:galaxy} \texttt{Galaxy} dataset. Kolmogorov--Smirnov distance $d_{KS}(\hat F_{\ell_M}, \hat F_{e_M})$ between estimated cdfs $\hat F_{\ell_M}$ and $\hat F_{e_M}$ under, respectively, the moment-match (with $\ell_M = 0.01$) and the relative error (with $e_M = 0.1, 0.05, 0.01$) criteria. The mixing measure of normal mixture is the \NGG with varying $\gamma\in\{0,0.25,0.5,0.75\}$.}
\end{table}
%\end{center} 
